Characterizing Task Completion Latencies in Fog Computing

Fog computing, which distributes computing resources to multiple locations between the Internet of Things (IoT) devices and the cloud, is attracting considerable attention from academia and industry. Yet, despite the excitement about the potential of fog computing, few comprehensive quantitative characteristics of the properties of fog computing architectures have been conducted. In this paper we examine the properties of task completion latencies in fog computing. First, we present the results of our empirical benchmarking-based study of task completion latencies. The study covered a range of settings, and uniquely considered both traditional and serverless fog computing execution points. It demonstrated the range of execution point characteristics in different locations and the relative stability of latency characteristics for a given location. It also highlighted properties of serverless execution that are not incorporated in existing fog computing algorithms. Second, we present a framework we developed for co-optimizing task completion quality and latency, which was inspired by the insights of our empirical study. We describe fog computing task assignment problems we formulated under this framework, and present the algorithms we developed for solving them.

==> Capacitated.tex <==
\begin{algorithm}[t]
\caption{Remove Cloud Assignments (RCA)}\label{alg:RCA}
\begin{algorithmic}[1]
\Procedure{RCA}{$J$}
\State $I_{jzx} \leftarrow$ UA($J$)
\State $p^{feas} \leftarrow 1, J^{plcd} \leftarrow \varnothing$
\For{$z: z \in Z$} \Comment{Check assignment's feasiblity}
    \State $C^{fld}_z \leftarrow \sum_{j} \sum_x I_{jzx}$
    \State \textbf{if} $C^{fld}_z>C_{z}$ \textbf{then} $p^{feas} \leftarrow 0$ \textbf{end if}
\EndFor
\State \textbf{if} $p^{feas}==1$ \textbf{then} $J^{plcd} \leftarrow J$ \textbf{end if}
\State \textbf{if} $p^{feas}\neq 1$ \textbf{then}
    \For{$z: z \in Z, C_z == \infty$}
        \For{$j: j \in J, z^*_j == z$}
                \State $J^{plcd} \leftarrow J^{plcd}\cup j$
        \EndFor
    \EndFor
\State \textbf{return} $\{p^{feas}, J^{plcd}$, $C^{fld}_z$ $\forall z\}$
%, $\{z^*_j, x^*_j, U^*_j \}\forall j$
\EndProcedure
\end{algorithmic}
\end{algorithm}

%\par
%\textbf{MG: look into the difference between multi-level and 2-level systems. There must be observations/lemmas that dramatically simplify the placement procedures for the 2-level systems. There must also be interesting properties of cases with infinite-capacity nodes}.

%The heuristics take into account that the capacity of some fog nodes can be infinite -- e.g., serverless nodes, -- while the capacity of others is restricted. They also take into account that some tasks have few placement options -- for example, as some of the placement options do not provide the sufficient response quality.

%\par
While the CTP is NP-hard in general, %% we have not actually demonstrated that, but we believe it to be true :) 
like other knapsack problems, for relatively small problem sizes it can be solved exactly~{kellerer2004knapsack}. 
\begin{itemize}
	\item In practical scenarios, problem size can be further reduced by placing tasks on the cloud. 
\end{itemize}


%% This is implemented in the script UtilityCalculations/PlacingTasksTwoTierArchitecture.m 
\par For the case of a capacitated gateway and an infinite-capacity cloud, we have a \emph{marginal-evaluation} algorithm that seems to be optimal. 
\begin{itemize}
	\item We are jointly solving admission control and placement problems. 
    \item We need to consider only one, best execution option on each node. %% This is easy to demonstrate 
	\item Place on the cloud what belongs on the cloud. That reduces the solution space. We called this the RCA procedure before. 
    \item For the other tasks, calculate the marginal gains from placing them on the gateway. The marginal gains are: the utility of placing the item on the gateway if the gateway is the only option (if there is no cloud option), or the difference between placing the item on the gateway and the cloud (if the cloud is an option). Pick the $C_{gat}$ items with the highest marginal gains, and place them on the gateway. 
    \item Among the remaining items, place those that we can on the gateway, and those that we cannot reject. 
    \item This is optimal why? 
    	\begin{itemize} 
        \item This is a knapsack problem with a single knapsack and all item weights being one. %% For the infinity variant, we "take" an item even if it does not appear in the knapsack? %% Seeing each item that can go on the cloud as a combination of two items? %% Needs more thinking 
        \item Lets denote $|J|$ by $T$
        \item Number of possible combinations, total: $T$ choose $C_{gat}$ = $T!$/$C_{gat}! \cdot (T-G_{gat}!)$.
       	\end{itemize}
    \item Complexity: $O$ remaining items. Quite a simple procedure. 
    \item Fairness could also be something to explore? 
    \item The approach naturally extends to many infinite-capacity options. For early tasks, place them where they belong on multiple infinite-capacity options. For later tasks, place them on the infinite-capacity option with the highest value. 
    \item This is evaluated with artificial data so far, but should work well with real data as well. 
\end{itemize} 

For two capacitated gateways: 
%% The script is UtilityCalculations/PlacingTasksTwoTierArchitectureTwoCapacitatedNodes.m
\begin{itemize}
	\item We calculate the marginals, over the cloud, for both gateways independently. 
    \item We use dynamic programming to calculate the optimal solution. Use a value iteration approach: 
    for each task $t = 1, ... T$, and each gateway fill level $c1 \in C1$ and $c2 \in C2$ %% notation abuse here, but whatever, lets get it done :) 
    $v(t,c1,c2)$ = $max$ of: 
    \begin{itemize} 
    \item $(v(t-1,c1-1,c2)+$value of the task $t$ placed on C1
    \item $(v(t-1,c1,c2-1)+$value of the task $t$ placed on C2
    \item $(v(t-1,c1,c2)$ -- this corresponds to rejecting the task
    \end{itemize}
   \item The complexity of this is $O(T \cdot C1 \cdot C2)$, which is reasonable for small $C1$ and $C2$. The $T$ here are only the tasks that have not been assigned to the cloud in the first pass-through. 
%     \item Then we order the tasks in order of the highest marginals. 
%     \item We pick the top choices for both gateways. 
%     \item This works well in general, but does not work where placing a task on either of the gateways is a good choice. Then by picking the one with the highest marginal, we can make a sub-optimal choice. 
%     	This is a myopic policy in this sense, picking the highest value. 
%         Can only happen if the same tasks are top picks on the different devices. 
    \item The weights of the picks are 1 on either gateway, but the benefit changes. We have two knapsacks -- this is a multiple knapsack formulation. 
    \item I believe the maximum number of combinations here is ($T$ choose $C_{gat1}) \cdot (T-C_{gat1})$ choose $C_{gat2}$. 
    \item For many capacitated gateways, the number of options is well-expressed in factorials: $T!/(C_1!\cdot C_2! \cdot ... \cdot (T-C_1-C_2 ...) !$. %% nice 
    	%Need to double-check this though. 
    \item This is a ``centralized'' version. We could draft a more solid distributed version as well. 
\end{itemize}


\begin{itemize}
\item Compare to others, e.g., to the case where we $\max$ individual tasks' quality levels? 
\end{itemize}


%The \textbf{Task-Shifting (TS)} heuristic is inspired by the structure of fog computing systems. 
% \begin{itemize}
% 	%\item Proposition: the TS is optimal for the case of a capacitated gateway and an infinite-capacity cloud (e.g., serverless cloud). Why: the assignments occupy no place on the cloud. This is something to try in practice. 
%     \item Proposition: the TS could be optimal for where we get non-zero utility for all placements of the tasks, given that we have infinite-capacity options. Need to experiment with it. 
% \end{itemize}

%The \textbf{Greedy-and-Swap (GNS)} heuristic is inspired by previously proposed approaches to multiple-choice multi-dimentional knapsack problems~\cite{hifi2004heuristic}. 


\par Both the TS and the GNS start by solving optimally the UTP obtained by relaxing Constr.~\ref{c:capacitated} in the CTP formulation. Then, in both TS and GNS the results of the UTP are processed with the Remove Cloud Assignments (RCA) procedure, detailed in Alg.~\ref{alg:RCA}, to check whether the relaxed UTP solution is a feasible solution to the original CTP. If feasible, the solution is also optimal, and the assignment completes. While usually the solution as a whole will not be feasible, solving the UTP identifies the tasks for which the best assignments are on fog nodes with $C_z = \infty$. \emph{Assigning these tasks for execution on these nodes is optimal for solving the CTP} (as we cannot improve on the assignments for these tasks, and making these assignments does not reduce the assignments options available to the other tasks). In the RCA we thus identify the optimal $\{z,x\}$ for the task subset $J^{plcd} \in J$; the next phases of both the TS and the GNS operate over a smaller set $J^{unpl} \buildrel\triangle\over = J \setminus J^{plcd}$.


\submissiononly{
\par
In the TS the output of the RCA is processed to identify $\{z \in Z: \sum_{j} \sum_{x} I_{jxz}>C_z\}$ (i.e., nodes for which Constr.~\ref{c:capacitated} is violated), and shift task assignments from these nodes to nodes with spare capacity ($\{z' \in Z: \sum_{j} \sum_{x} I_{jxz}<C_z\}$). In choosing the specific task shifts out of all shifts possible, the TS minimizes the loss of the total utility of task assignments. The TS is straightforward and is a good match to settings where only some nodes have tight capacity restrictions (e.g., where consumer electronics-grade fog nodes can serve few tasks).
However, the TS does not always find a feasible solution where one exists. For the cases where the TS cannot find a solution, the GNS can be used following the TS.\footnote{The pseudocode for the post-RCA phases of both the TS and the GNS is available in the technical report~\cite{CaaSReportAnon2017}.}
}


